Self-Reorganizing and Rejuvenating CNNs for Increasing Model Capacity Utilization

In this paper, we propose self-reorganizing and rejuvenating convolutional neural networks; a biologically inspired method for improving the computational resource utilization of neural networks. The proposed method utilizes the channel activations of a convolution layer in order to reorganize that layers parameters. The reorganized parameters are clustered to avoid parameter redundancies. As such, redundant neurons with similar activations are merged leaving room for the remaining parameters to rejuvenate. The rejuvenated parameters learn different features to supplement those learned by the reorganized surviving parameters. As a result, the network capacity utilization increases improving the baseline network performance without any changes to the network structure. The proposed method can be applied to various network architectures during the training stage, or applied to a pre-trained model improving its performance. Experimental results showed that the proposed method is model-agnostic and can be applied to any backbone architecture increasing its performance due to the elevated utilization of the network capacity.

==> sections/04-01-exp1.tex <==
In this experiments, we demonstrate the effectiveness of the proposed self-reorganizing and rejuvenating CNNs on improving the performance of over-parameterized baseline models. To assure that the baseline models are over-parameterized, two types of experiments were performed. First, experiments were performed on CIFAR-100 dataset using architectures that are well known to perform well on Imagenet dataset. Since the classification using the CIFAR-100 dataset is a simpler task compared to Imagenet classification, models that are known to work well on Imagenet can be considered over-parametrized when used on the CIFAR-100 dataset. The second type of experiments was done using deep models on the Imagenet dataset. In both experiments, the proposed method was applied to the last convolutional layer of the architecture, and the performance was recorded accordingly. 

For the CIFAR-100 experiments, AlexNet \cite{alexnet}, MobileNet \cite{mobilenet}, ResNet-18 and ResNet-50 \cite{resnet}  has been utilized. Some minor changes have been applied to the AlexNet and the ResNet models, in order to adjust them to the CIFAR-100 dataset. In the AlexNet baseline model, local response normalization has been replaced with batch normalization, and the convolution kernels of the first and second layers have been set to $3\times3$ as in \cite{dorefa}. The ResNet models were modified such that the kernel of the first layer has been set to $3\times3$. In the neuron reorganization stage of the proposed method, the size of the SOFM was set to 50\% of the output channels of the last convolutional layer. By doing so, all the parameters of the layer are reorganized to half the size of the original layer. The remaining 50\% of the parameters were randomly reinitialized. Table ~\ref{Table:1} shows the results of applying the proposed method with comparison to the baseline models. For comparison, two other rejuvenation techniques were also trained and recorded in Table~\ref{Table:1}. The first model ($\ell_2$), is similar to the DSD \cite{dsd} approach by relying on $ \|  \mathbf{\widetilde{W}}^{(l)} \|_2$. In particular, we  obtained the $\ell_2$ norm of the weights ($ \|  \mathbf{\widetilde{W}}^{(l)} \|_2$), then the lowest 50\% of the $\ell_2$ norms was reinitialized and rejuvenated by training the model end-to-end. The second method ($\ell_1$) is influenced by \cite{NR}, in the fact that it applies a sparsity constraint on the standard deviation parameter of the batch-norm layer $(\gamma)$.  Then, the lowest 50\% of the $|  \mathbf{\gamma}^{(l)} |$ was reinitialized and rejuvenated by training the model end-to-end. Note that, in the comparative methods 50\% was reinitialized for a fair comparison with the proposed method. The results in Table~\ref{Table:1} show that the proposed method outperformes the baseline and the comparative methods.  Note that, since the comparative methods and the proposed method reinitialize the same percentage of the parameters. Yet, the proposed method was able to achieve the most performance gain.  This shows that the performance gain is not due to the re-initialization of the parameters. The proposed method was able to project the layer parameteres into a compressed space, then, rejuvenate and extend the capacity of that model improving its performance. 


The results on the Imagenet dataset are shown in Table~\ref{Table:2}. As baseline models, DenseNet-121 \cite{densenet}, ResNet-50, ResNet-101 and ResNet-152 \cite{resnet} were utilized. For comparison, the results of neuron rejuvenation when adding a constraint on the number of parameters \cite{NR} were also reported.  The results in Table~\ref{Table:2} show that the proposed method outperform the baseline and \cite{NR}. More interestingly, the larger the model the more performance gain was obtained, since larger models tend to be more over-parameterized. It could also be seen from Table~\ref{Table:2} that the performance of self reorganized smaller models becomes comparable with larger models (e.g. self-reorganized and rejuvenated ResNet-101 compared to ResNet-152 baseline). This testifies that the proposed method better utilizes the capacity of the model.Finally, the results in Table~\ref{Table:1} and Table~\ref{Table:2} also show that the proposed method is model-agnostic and can work with different baseline models. 



%The results on the Imagenet dataset are shown in Table~\ref{Table:2}. As baseline models, DenseNet-121 \cite{densenet}, ResNet-50, ResNet-101 and ResNet-152 \cite{resnet} were utilized. As in the CIFAR-100 experiments, the proposed method was applied to the last layer. However, in the neuron reorganization stage of the proposed method, the size of the SOFM was set to 75\% of the output channels of the last convolutional layer. As expected the proposed method outperformed the baseline method. More interestingly, the larger the model the more performance improvement was gained. This testifies to the fact that the proposed method better utilizes the capacity of the model, since larger models tend to be more over-parameterized.

